Luminosities and infrared excess in Type II and anomalous Cepheids in the Large and Small Magellanic Clouds

(abridged) Type II and anomalous Cepheids (ACs) are useful distance indicators when there are too few classical Cepheids or when RR Lyrae stars are too faint. We study the sample of 335 Type II and ACs in the Small and Large MCls detected in OGLE-III data.The SEDs are constructed and fitted with a dust radiative transfer model, thereby leading to a determination of luminosity and effective temperature.In addition, a subsample of targets is investigated for possible binarity by looking for the light-time travel effect (LITE). Hertzsprung-Russell diagrams (HRD) are constructed and compared to evolutionary tracks and theoretical instability strips (ISs). In agreement with previous suggestions, the BL Her subclass can be explained by the evolution of $\sim$0.5-0.6~\msol\ stars evolving off the ZAHB and the ACs can be explained by the evolution of $\sim$1.1-2.3~\msol\ stars. The evolution of the W Vir subclass is not clear. A relation to binarity might be at the origin of the W Vir stars, which has already been explicitly suggested for the peculiar W Vir stars. For $\sim60\%$ of the RV Tau and $\sim 10\%$ of the W Vir objects an infrared excess is detected from the SED fitting. A recent result is confirmed that stars exist with luminosities below that predicted from single-star evolution, which show a clear infrared excess, and the shape of the excess suggests a connection to binary evolution. The investigation of the LITE effect revealed 20 systems that appear to show periodic variations and may be new binaries, although this study requires follow-up. About 40 stars show significant period changes.

==> TabA1.tex <==
OGLE-LMC-ACEP-001   ANCEP  F        0.850    78    3  6125  188  0.000  1000  0    
OGLE-LMC-ACEP-002   ANCEP  F        0.977   119    5  6250  188  0.000  1000  0    
OGLE-LMC-ACEP-003   ANCEP  1O       0.382    66    2  6750  250  0.000  1000  0    
OGLE-LMC-ACEP-004   ANCEP  F        1.862   200   17  6000  812  0.000  1000  0    
OGLE-LMC-ACEP-005   ANCEP  F        0.932    92    1  6125  188  0.000  1000  0    
OGLE-LMC-ACEP-006   ANCEP  1O       0.850   200    5  6250  188  0.000  1000  0    
OGLE-LMC-ACEP-007   ANCEP  F        0.896   114    4  6375  250  0.000  1000  0    
OGLE-LMC-ACEP-008   ANCEP  1O       0.749   168    5  6375  125  0.000  1000  0    
OGLE-LMC-ACEP-009   ANCEP  1O       0.800   153    3  6250  125  0.000  1000  0    
OGLE-LMC-ACEP-010   ANCEP  F        0.834    81    3  6250  312  0.000  1000  0    
OGLE-LMC-ACEP-011   ANCEP  F        0.999   118    7  5625  250  0.000  1000  0    
OGLE-LMC-ACEP-012   ANCEP  F        0.829   107   12  5875 1062  0.000  1000  0    
OGLE-LMC-ACEP-013   ANCEP  1O       0.501    77    3  6250  500  0.000  1000  0    
OGLE-LMC-ACEP-014   ANCEP  F        2.291   299    7  6125  125  0.000  1000  0    
OGLE-LMC-ACEP-015   ANCEP  1O       1.181   218    4  6375  188  0.000  1000  0    
OGLE-LMC-ACEP-016   ANCEP  F        1.546   214    9  6250  188  0.000  1000  0    
OGLE-LMC-ACEP-017   ANCEP  F        0.930   127    3  6250  125  0.000  1000  0    
OGLE-LMC-ACEP-018   ANCEP  F        1.019   124    4  6500  312  0.000  1000  0    
OGLE-LMC-ACEP-019   ANCEP  F        0.909   159    3  6750  188  0.000  1000  0    
OGLE-LMC-ACEP-020   ANCEP  1O       0.382   100    4  7375  312  0.000  1000  0    
OGLE-LMC-ACEP-021   ANCEP  F        1.296   159    7  6125  562  0.000  1000  0    
OGLE-LMC-ACEP-023   ANCEP  1O       0.723   190    9  6375  188  0.000  1000  0    
OGLE-LMC-ACEP-024   ANCEP  F        0.794   139    3  7500  125  0.000  1000  0    
OGLE-LMC-ACEP-025   ANCEP  1O       0.474   100    6  7000  500  0.000  1000  0    
OGLE-LMC-ACEP-026   ANCEP  F        1.739   228    3  5875  125  0.000  1000  0    
OGLE-LMC-ACEP-027   ANCEP  F        1.267   222   10  6500  312  0.000  1000  0    
OGLE-LMC-ACEP-028   ANCEP  1O       0.599   111    5  5375  312  0.000  1000  0    
OGLE-LMC-ACEP-029   ANCEP  F        0.802    77    2  6625  250  0.000  1000  0    
OGLE-LMC-ACEP-030   ANCEP  1O       0.667   173    6  6500  250  0.000  1000  0    
OGLE-LMC-ACEP-031   ANCEP  1O       0.840   167    7  6375  438  0.000  1000  0    
OGLE-LMC-ACEP-032   ANCEP  F        1.316   174    4  6000  125  0.000  1000  0    
OGLE-LMC-ACEP-033   ANCEP  F        2.347   294    5  6000  125  0.000  1000  0    
OGLE-LMC-ACEP-034   ANCEP  F        0.734    96    8  6375  812  0.000  1000  0    
OGLE-LMC-ACEP-035   ANCEP  1O       0.446    76    1  6625  125  0.000  1000  0    
OGLE-LMC-ACEP-036   ANCEP  F        1.258   170    3  6000  125  0.000  1000  0    
OGLE-LMC-ACEP-037   ANCEP  F        1.258   258   17  5125  375  0.000  1000  0    
OGLE-LMC-ACEP-038   ANCEP  F        1.335   164    4  6375  188  0.000  1000  0    
OGLE-LMC-ACEP-039   ANCEP  F        0.992   115    1  6375   62  0.000  1000  0    
OGLE-LMC-ACEP-040   ANCEP  F        0.961   136    5  6000  375  0.000  1000  0    
OGLE-LMC-ACEP-041   ANCEP  F        0.878   101    7  6250  688  0.000  1000  0    
OGLE-LMC-ACEP-042   ANCEP  F        1.079    82    3  5000  125  0.000  1000  0    
OGLE-LMC-ACEP-043   ANCEP  1O       0.506    85    1  6000  125  0.000  1000  0    
OGLE-LMC-ACEP-044   ANCEP  F        1.309   229   11  6750  312  0.000  1000  0    
OGLE-LMC-ACEP-045   ANCEP  F        0.678    59    1  6125  250  0.000  1000  0    
OGLE-LMC-ACEP-046   ANCEP  F        1.264   179   11  6375  500  0.000  1000  0    
OGLE-LMC-ACEP-047   ANCEP  F        2.178   237    8  6375  188  0.000  1000  0    
OGLE-LMC-ACEP-048   ANCEP  F        1.546   230   12  6000  438  0.000  1000  0    
OGLE-LMC-ACEP-049   ANCEP  F        0.645    89    6  6875  562  0.000  1000  0    
OGLE-LMC-ACEP-050   ANCEP  1O       1.045   335    9  6750  125  0.000  1000  0    
OGLE-LMC-ACEP-051   ANCEP  F        0.709    68    1  6125   62  0.000  1000  0    
OGLE-LMC-ACEP-052   ANCEP  F        1.263   191    9  6125  312  0.000  1000  0    
OGLE-LMC-ACEP-053   ANCEP  F        1.888   267   12  5750  375  0.000  1000  0    
OGLE-LMC-ACEP-054   ANCEP  F        0.980    82    2  5375  188  0.000  1000  0    
OGLE-LMC-ACEP-055   ANCEP  F        1.607   188   10  5875  375  0.000  1000  0    
OGLE-LMC-ACEP-056   ANCEP  F        1.124   144    7  6125  500  0.000  1000  0    
OGLE-LMC-ACEP-057   ANCEP  F        1.710   250    6  6000  188  0.000  1000  0    
OGLE-LMC-ACEP-058   ANCEP  1O       0.485   142    9  7875  812  0.000  1000  0    
OGLE-LMC-ACEP-059   ANCEP  F        0.835    42    2  4500  188  0.000  1000  0    
OGLE-LMC-ACEP-060   ANCEP  F        1.276   221    4  6375  250  0.000  1000  0    
OGLE-LMC-ACEP-061   ANCEP  F        0.848    99    2  6125  188  0.000  1000  0    
OGLE-LMC-ACEP-062   ANCEP  F        1.059   216   14  7000  500  0.000  1000  0    
OGLE-LMC-ACEP-063   ANCEP  F        0.893    70    2  5625  250  0.000  1000  0    
OGLE-LMC-ACEP-064   ANCEP  F        1.357   203    4  6250  250  0.000  1000  0    
OGLE-LMC-ACEP-065   ANCEP  F        1.322   195   10  6500  438  0.000  1000  0    
OGLE-LMC-ACEP-066   ANCEP  F        1.040   124    3  6250  250  0.000  1000  0    
OGLE-LMC-ACEP-067   ANCEP  F        0.821   101   11  5750 1125  0.000  1000  0    
OGLE-LMC-ACEP-068   ANCEP  F        0.626    65    5  6875  562  0.000  1000  0   IR excess?  
OGLE-LMC-ACEP-069   ANCEP  F        1.538   254    7  5875  250  0.000  1000  0    
OGLE-LMC-ACEP-070   ANCEP  1O       0.629    98    3  6500  312  0.000  1000  0    
OGLE-LMC-ACEP-071   ANCEP  1O       0.676   171   10  7125  375  0.000  1000  0    
OGLE-LMC-ACEP-072   ANCEP  F        1.048   201    8  6500  375  0.000  1000  0    
OGLE-LMC-ACEP-073   ANCEP  F        1.465   255   11  6375  438  0.000  1000  0    
OGLE-LMC-ACEP-074   ANCEP  F        1.533   221    4  6250  188  0.000  1000  0    
OGLE-LMC-ACEP-075   ANCEP  F        0.692    88    3  6500  312  0.000  1000  0    
OGLE-LMC-ACEP-076   ANCEP  F        1.582   193    5  6250  312  0.000  1000  0    
OGLE-LMC-ACEP-077   ANCEP  F        1.122   129    5  5875  125  0.000  1000  0    
OGLE-LMC-ACEP-078   ANCEP  1O       0.857   236    5  6875  188  0.000  1000  0    
OGLE-LMC-ACEP-079   ANCEP  F        1.155   202   10  6625  250  0.000  1000  0    
OGLE-LMC-ACEP-080   ANCEP  F        1.057   143    3  6375  250  0.000  1000  0    
OGLE-LMC-ACEP-081   ANCEP  F        0.801    89    3  6375  188  0.000  1000  0    
OGLE-LMC-ACEP-082   ANCEP  1O       0.775   154    3  5625  125  0.000  1000  0    
OGLE-LMC-T2CEP-001  T2CEP  BLHer    1.814   101    1  6000   62  0.000  1000  0    
OGLE-LMC-T2CEP-002  T2CEP  WVir    18.324   629   29  5250  312  0.000  1000  0    
OGLE-LMC-T2CEP-003  T2CEP  RVTau   35.660  4228  191  6000  438  1.382  1300  0    
OGLE-LMC-T2CEP-004  T2CEP  BLHer    1.916   143   12  5625  438  0.000  1000  0    
OGLE-LMC-T2CEP-005  T2CEP  RVTau   33.185  1277  136  4875  312  0.000  1000  0    
OGLE-LMC-T2CEP-006  T2CEP  BLHer    1.088    84    3  7000  312  0.000  1000  0    
OGLE-LMC-T2CEP-007  T2CEP  BLHer    1.243    87    3  6750  250  0.000  1000  0    
OGLE-LMC-T2CEP-008  T2CEP  BLHer    1.746    90    2  5875  125  0.000  1000  0    
OGLE-LMC-T2CEP-009  T2CEP  BLHer    1.761   104    2  6250  125  0.000  1000  0    
OGLE-LMC-T2CEP-010  T2CEP  BLHer    1.503    87    2  6500  250  0.000  1000  0    
OGLE-LMC-T2CEP-011  T2CEP  RVTau   39.257  2893   61  5875  125  0.045   906  1    
OGLE-LMC-T2CEP-012  T2CEP  WVir    11.581   419   13  5250  250  0.000  1000  0    
OGLE-LMC-T2CEP-013  T2CEP  WVir    11.545   388    8  5250  125  0.000  1000  0    
OGLE-LMC-T2CEP-014  T2CEP  RVTau   61.876  2325   52  5750  125  0.078  1100  0    
OGLE-LMC-T2CEP-015  T2CEP  RVTau   56.521  2910   53  5000  125  0.261  1200  0  P=56.224 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-016  T2CEP  RVTau   20.296  1025   54  6750  312  0.122   600  0    
OGLE-LMC-T2CEP-017  T2CEP  WVir    14.455   476   19  4875  188  0.000  1000  0    
OGLE-LMC-T2CEP-018  T2CEP  BLHer    1.380    88    1  6375  125  0.000  1000  0    
OGLE-LMC-T2CEP-019  T2CEP  pWVir    8.675   436   35  5000  750  0.000  1000  0    
OGLE-LMC-T2CEP-020  T2CEP  BLHer    1.108    93    4  6500  312  0.000  1000  0    
OGLE-LMC-T2CEP-021  T2CEP  pWVir    9.760   552   14  5750  125  0.000  1000  0  EB  
OGLE-LMC-T2CEP-022  T2CEP  WVir    10.717   383    8  5250  188  0.000  1000  0  W3 excess  
OGLE-LMC-T2CEP-023  T2CEP  pWVir    5.235   837   26  6250  250  0.000  1000  0  EB  
OGLE-LMC-T2CEP-024  T2CEP  BLHer    1.247    75    3  6500  375  0.000  1000  0    
OGLE-LMC-T2CEP-025  T2CEP  RVTau   67.965  2911  179  4875  312  0.000  1000  0  IR excess?   
OGLE-LMC-T2CEP-026  T2CEP  WVir    13.578   443   10  5000  125  0.000  1000  0    
OGLE-LMC-T2CEP-027  T2CEP  WVir    17.134   619   25  5500  375  0.000  1000  0  P=17.127 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-028  T2CEP  pWVir    8.785   833   36  6375  375  0.000  1000  0    
OGLE-LMC-T2CEP-029  T2CEP  RVTau   31.245  2851   79  5750  188  1.347   746  1  P=31.716 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-030  T2CEP  BLHer    3.935   202    5  5750  125  0.000  1000  0    
OGLE-LMC-T2CEP-031  T2CEP  WVir     6.706   253    4  5375  125  0.000  1000  0    
OGLE-LMC-T2CEP-032  T2CEP  RVTau   44.561  3821  590  4625 1000  1.763   800  0    
OGLE-LMC-T2CEP-033  T2CEP  pWVir    9.395   605   14  5875  250  0.000  1000  0  P=9.387 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-034  T2CEP  WVir    14.911   411   14  4750  125  0.000  1000  0  P=14.906 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-035  T2CEP  WVir     9.866   384   16  5000  250  0.000  1000  0    
OGLE-LMC-T2CEP-036  T2CEP  WVir    14.881   501   17  5625  188  0.000  1000  0    
OGLE-LMC-T2CEP-037  T2CEP  WVir     6.897   266    4  5625  125  0.000  1000  0    
OGLE-LMC-T2CEP-038  T2CEP  WVir     4.014   537   28  7250  375  0.000  1000  0    
OGLE-LMC-T2CEP-039  T2CEP  WVir     8.716   367   13  5625  250  0.000  1000  0  W3 excess  
OGLE-LMC-T2CEP-040  T2CEP  pWVir    9.626   639   31  5000  375  0.000  1000  0  P=9.622 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-041  T2CEP  BLHer    2.476   290   16  7250  562  0.000  1000  0    
OGLE-LMC-T2CEP-042  T2CEP  pWVir    4.923   384   23  6750  562  0.000  1000  0    
OGLE-LMC-T2CEP-043  T2CEP  WVir     6.559   211    5  5375  188  0.000  1000  0    
OGLE-LMC-T2CEP-044  T2CEP  WVir    13.270   439    9  5250  188  0.000  1000  0  P=13.246 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-045  T2CEP  RVTau   63.386  3479  130  5125  125  0.000  1000  0  IR excess?  
OGLE-LMC-T2CEP-046  T2CEP  WVir    14.744   879   21  5250  125  0.718   809  1  P=14.752 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-047  T2CEP  WVir     7.286   285    7  5500  250  0.000  1000  0    
OGLE-LMC-T2CEP-048  T2CEP  BLHer    1.445    92    8  6375  812  0.000  1000  0    
OGLE-LMC-T2CEP-049  T2CEP  BLHer    3.235   231   19  6375  812  0.000  1000  0    
OGLE-LMC-T2CEP-050  T2CEP  RVTau   34.748  1427   34  5875  125  0.117  1200  0    
OGLE-LMC-T2CEP-051  T2CEP  RVTau   40.606  1850   49  5500  188  0.000  1000  0    
OGLE-LMC-T2CEP-052  T2CEP  pWVir    4.688   448   29  7000  500  0.000  1000  0  EB  
OGLE-LMC-T2CEP-053  T2CEP  BLHer    1.043    81    2  6625  188  0.000  1000  0    
OGLE-LMC-T2CEP-054  T2CEP  WVir     9.925   338    4  5125   62  0.000  1000  0    
OGLE-LMC-T2CEP-055  T2CEP  RVTau   41.005  2545   77  5750  188  0.080  1000  0    
OGLE-LMC-T2CEP-056  T2CEP  WVir     7.290   246    3  5125   62  0.000  1000  0    
OGLE-LMC-T2CEP-057  T2CEP  WVir    16.632   569   19  5125  312  0.000  1000  0  P=16.602 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-058  T2CEP  RVTau   21.483   715   24  5125  312  0.000  1000  0  P=21.486 [1998AJ....115.1921A] 
OGLE-LMC-T2CEP-059  T2CEP  WVir    16.736   720   26  5125  250  0.000  1000  0  P=16.747 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-060  T2CEP  BLHer    1.237    73    4  6250  688  0.000  1000  0    
OGLE-LMC-T2CEP-061  T2CEP  BLHer    1.182    82    5  7125  562  0.000  1000  0    
OGLE-LMC-T2CEP-062  T2CEP  WVir     6.047   190   19  4750  438  0.000  1000  0    
OGLE-LMC-T2CEP-063  T2CEP  WVir     6.925   278    8  5625  250  0.000  1000  0    
OGLE-LMC-T2CEP-064  T2CEP  BLHer    2.128   121    8  6125  750  0.000  1000  0    
OGLE-LMC-T2CEP-065  T2CEP  RVTau   35.055  1563   20  5375  125  0.100   120  0    
OGLE-LMC-T2CEP-066  T2CEP  WVir    13.109   412    6  5125   62  0.000   500  0    
OGLE-LMC-T2CEP-067  T2CEP  RVTau   48.232  6429  305  6125  500  1.743  1200  0  P=48.539 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-068  T2CEP  BLHer    1.609   106    2  6500  250  0.000  1000  0    
OGLE-LMC-T2CEP-069  T2CEP  BLHer    1.021    93   14  6625 1062  0.000  1000  0    
OGLE-LMC-T2CEP-070  T2CEP  WVir    15.438   675   36  5875  312  0.000  1000  0  W3 excess   
OGLE-LMC-T2CEP-071  T2CEP  BLHer    1.152    76    9  6375  875  0.000  1000  0    
OGLE-LMC-T2CEP-072  T2CEP  WVir    14.514   534   11  5375  125  0.000  1000  0    
OGLE-LMC-T2CEP-073  T2CEP  BLHer    3.088   169    5  5875  250  0.000  1000  0    
OGLE-LMC-T2CEP-074  T2CEP  WVir     8.988   456    9  5625  188  0.000  1000  0    
OGLE-LMC-T2CEP-075  T2CEP  RVTau   50.187  1868   68  5125  125  0.087   646  1  
OGLE-LMC-T2CEP-076  T2CEP  BLHer    2.104    89    3  5500  312  0.000  1000  0    
OGLE-LMC-T2CEP-077  T2CEP  BLHer    1.214   132    5  7500  375  0.000  1000  0  EB  
OGLE-LMC-T2CEP-078  T2CEP  pWVir    6.716   404   14  4875  125  0.000  1000  0    
OGLE-LMC-T2CEP-079  T2CEP  WVir    14.845   344   19  4875  188  0.000  1000  0  P=14.855 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-080  T2CEP  RVTau   40.916  2395  104  5625  250  0.113   331  1  P=41.118 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-081  T2CEP  WVir     9.480   369    7  5375  125  0.000  1000  0    
OGLE-LMC-T2CEP-082  T2CEP  RVTau   35.124  1127   75  5125  312  0.000  1000  0    
OGLE-LMC-T2CEP-083  T2CEP  pWVir    5.968   284    6  5625  125  0.000  1000  0    
OGLE-LMC-T2CEP-084  T2CEP  BLHer    1.771   260   40  7750 1562  0.000  1000  0  EB   
OGLE-LMC-T2CEP-085  T2CEP  BLHer    3.405   177    6  6250  375  0.000  1000  0    
OGLE-LMC-T2CEP-086  T2CEP  WVir    15.845   665   15  5500  188  0.000  1000  0    
OGLE-LMC-T2CEP-087  T2CEP  WVir     5.185   213    9  5500  438  0.000  1000  0    
OGLE-LMC-T2CEP-088  T2CEP  BLHer    1.951   223   11  8000  375  0.000  1000  0    
OGLE-LMC-T2CEP-089  T2CEP  BLHer    1.167    88    2  6750  188  0.000  1000  0    
OGLE-LMC-T2CEP-090  T2CEP  BLHer    1.479    96    2  6250  250  0.000  1000  0    
OGLE-LMC-T2CEP-091  T2CEP  RVTau   35.749  3880  319  6625  625  1.259  1100  0    
OGLE-LMC-T2CEP-092  T2CEP  BLHer    2.617   133    7  6000  625  0.000  1000  0    
OGLE-LMC-T2CEP-093  T2CEP  WVir    17.593  1211   46  5875  250  0.000  1000  0  EB, P=17.560 [1998AJ....115.1921A], P=17.68586 [2002ApJ...573..338A] 
OGLE-LMC-T2CEP-094  T2CEP  WVir     8.468   285    8  5000  125  0.000  1000  0    
OGLE-LMC-T2CEP-095  T2CEP  WVir     5.000   187    3  5375   62  0.000  1000  0    
OGLE-LMC-T2CEP-096  T2CEP  WVir    13.926   498   15  5375  312  0.000  1000  0  P=13.925 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-097  T2CEP  WVir    10.510   423   10  5500  250  0.000  1000  0  P=10.509 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-098  T2CEP  pWVir    4.974  2857  169  7375  312  0.000  1000  0  EB, P=4.97371 [2002ApJ...573..338A]  
OGLE-LMC-T2CEP-099  T2CEP  WVir    15.487   516   17  4625  188  0.000  1000  0    
OGLE-LMC-T2CEP-100  T2CEP  WVir     7.431   265    5  5875  188  0.000  1000  0    
OGLE-LMC-T2CEP-101  T2CEP  WVir    11.419   499   17  5875  375  0.000  1000  0  P=11.442 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-102  T2CEP  BLHer    1.266   115    5  6875  438  0.000  1000  0    
OGLE-LMC-T2CEP-103  T2CEP  WVir    12.908   454   12  5375  250  0.000  1000  0  P=12.902 [1998AJ....115.1921A]   
OGLE-LMC-T2CEP-104  T2CEP  RVTau   24.880  1889   54  5500  438  1.168  1100  0  P=24.848 [1998AJ....115.1921A]   
OGLE-LMC-T2CEP-105  T2CEP  BLHer    1.489   117    6  6500  625  0.000  1000  0    
OGLE-LMC-T2CEP-106  T2CEP  WVir     6.707   272    6  5500  188  0.000  1000  0    
OGLE-LMC-T2CEP-107  T2CEP  BLHer    1.209   105    5  5875  562  0.000  1000  0    
OGLE-LMC-T2CEP-108  T2CEP  RVTau   30.011  1654   37  5750  125  0.000  1000  0    
OGLE-LMC-T2CEP-109  T2CEP  BLHer    1.415    18    1  4125  112  0.000  1000  0    
OGLE-LMC-T2CEP-110  T2CEP  WVir     7.078   242    7  5250  250  0.000  1000  0    
OGLE-LMC-T2CEP-111  T2CEP  WVir     7.496   289    5  5500  125  0.000  1000  0    
OGLE-LMC-T2CEP-112  T2CEP  RVTau   39.398  3186  137  6000  188  0.091  1200  0    
OGLE-LMC-T2CEP-113  T2CEP  BLHer    3.085   267   26  6625  688  0.000  1000  0    
OGLE-LMC-T2CEP-114  ANCEP  F        1.091    68    1  5250  188  0.000  1000  0  [2015AcA....65..233S]
OGLE-LMC-T2CEP-115  T2CEP  RVTau   24.967   768   29  5000  188  0.000  1000  0  P=24.935 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-116  T2CEP  BLHer    1.967    79    3  5500  312  0.000  1000  0    
OGLE-LMC-T2CEP-117  T2CEP  WVir     6.629   258    6  5500  125  0.000  1000  0    
OGLE-LMC-T2CEP-118  T2CEP  WVir    12.699   428   12  5125  188  0.000  1000  0  P=12.704 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-119  T2CEP  RVTau   33.825  3325  290  6250  625  1.440  1200  0    
OGLE-LMC-T2CEP-120  T2CEP  WVir     4.559   185    4  5500  188  0.000  1000  0    
OGLE-LMC-T2CEP-121  T2CEP  BLHer    2.061   104    5  5875  562  0.000  1000  0    
OGLE-LMC-T2CEP-122  T2CEP  BLHer    1.539    63    2  5750  312  0.000  1000  0    
OGLE-LMC-T2CEP-123  T2CEP  BLHer    1.003    84    8  5000  438  0.000  1000  0    
OGLE-LMC-T2CEP-124  T2CEP  BLHer    1.735    83    4  6000  438  0.000  1000  0    
OGLE-LMC-T2CEP-125  T2CEP  RVTau   33.034  1208   53  5125  250  0.000  1000  0  IR excess?  
OGLE-LMC-T2CEP-126  T2CEP  WVir    16.327   467   26  4750  125  0.981   313  1    
OGLE-LMC-T2CEP-127  T2CEP  WVir    12.669   536   62  5500  500  0.305   363  1    
OGLE-LMC-T2CEP-128  T2CEP  WVir    18.493   834   38  5125  250  0.000  1000  0    
OGLE-LMC-T2CEP-129  T2CEP  RVTau   62.509  3132   80  6000  125  0.091   700  0    
OGLE-LMC-T2CEP-130  T2CEP  BLHer    1.945   123    8  6375  688  0.000  1000  0    
OGLE-LMC-T2CEP-131  T2CEP  BLHer    1.413    65    1  6000  125  0.000  1000  0    
OGLE-LMC-T2CEP-132  T2CEP  pWVir   10.018   540   17  5625  312  0.000  1000  0    
OGLE-LMC-T2CEP-133  T2CEP  WVir     6.282   269    7  5750  250  0.000  1000  0    
OGLE-LMC-T2CEP-134  T2CEP  pWVir    4.076   406    8  6125  250  0.000  1000  0    
OGLE-LMC-T2CEP-135  T2CEP  RVTau   26.522  1047   24  5000  188  0.000  1000  0   P=26.594 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-136  T2CEP  BLHer    1.323   163   21  5625 1188  0.000  1000  0    
OGLE-LMC-T2CEP-137  T2CEP  WVir     6.362   265    9  5625  375  0.000  1000  0    
OGLE-LMC-T2CEP-138  T2CEP  BLHer    1.394    79   12  5375 1312  0.000  1000  0    
OGLE-LMC-T2CEP-139  T2CEP  WVir    14.780   484   13  5000  125  0.000  1000  0    
OGLE-LMC-T2CEP-140  T2CEP  BLHer    1.841   103    3  6000  312  0.000  1000  0    
OGLE-LMC-T2CEP-141  T2CEP  BLHer    1.823    73    3  5875  438  0.000  1000  0    
OGLE-LMC-T2CEP-142  T2CEP  BLHer    1.761   108    2  5500   62  0.000  1000  0    
OGLE-LMC-T2CEP-143  T2CEP  WVir    14.570   548   18  5750  312  0.000  1000  0    
OGLE-LMC-T2CEP-144  T2CEP  BLHer    1.937   103   26  5375 1312  0.000  1000  0    
OGLE-LMC-T2CEP-145  T2CEP  BLHer    3.337   267   21  6500  688  0.000  1000  0    
OGLE-LMC-T2CEP-146  T2CEP  WVir    10.080   298   11  5000  188  0.000  1000  0    
OGLE-LMC-T2CEP-147  T2CEP  RVTau   46.796  7160  259  6375  312  1.528   621  1  P=46.542 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-148  T2CEP  BLHer    2.672   135    4  6250  250  0.000  1000  0    
OGLE-LMC-T2CEP-149  T2CEP  RVTau   42.481  2741  117  5750  250  0.000  1000  0  P=42.079 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-150  T2CEP  WVir     5.493   496    9  6500  125  0.152  1100  0    
OGLE-LMC-T2CEP-151  T2CEP  WVir     7.887   311    7  5500  250  0.000  1000  0    
OGLE-LMC-T2CEP-152  T2CEP  WVir     9.315   356   12  5250  312  0.000  1000  0  P=9.309 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-153  T2CEP  BLHer    1.175   465   19  8000  250  0.000  1000  0    
OGLE-LMC-T2CEP-154  T2CEP  pWVir    7.578  1071   28  6750  125  0.000  1000  0    
OGLE-LMC-T2CEP-155  T2CEP  WVir     6.898   282   13  5000  438  0.000  1000  0    
OGLE-LMC-T2CEP-156  T2CEP  WVir    15.387   581   79  4875  188  0.530   151  1  P=15.391 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-157  T2CEP  WVir    14.335   431   10  5000  125  0.000  1000  0  P=14.337 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-158  T2CEP  WVir     7.139   270    9  5500  188  0.150   300  0    
OGLE-LMC-T2CEP-159  T2CEP  WVir     6.626   221    3  5125   62  0.000  1000  0    
OGLE-LMC-T2CEP-160  T2CEP  BLHer    1.757    90    3  5875  375  0.000  1000  0    
OGLE-LMC-T2CEP-161  T2CEP  WVir     8.532   548   26  5125  312  0.000  1000  0    
OGLE-LMC-T2CEP-162  T2CEP  RVTau   30.394  1109   44  5000  188  0.183  1000  0  P=30.408 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-163  T2CEP  BLHer    1.694   140   16  6250  875  0.000  1000  0    
OGLE-LMC-T2CEP-164  T2CEP  pWVir    8.495   550   14  5500  250  0.483  1300  0    
OGLE-LMC-T2CEP-165  T2CEP  BLHer    1.241    35    1  4875  125  0.000  1000  0    
OGLE-LMC-T2CEP-166  T2CEP  BLHer    2.111   211    7  5625  312  0.000  1000  0    
OGLE-LMC-T2CEP-167  T2CEP  BLHer    2.312    99    4  5375  438  0.000  1000  0    
OGLE-LMC-T2CEP-168  T2CEP  WVir    15.698   554   15  5250  125  0.000  1000  0    
OGLE-LMC-T2CEP-169  T2CEP  RVTau   30.956  1893  379  6250  625  0.442   477  1  P=31.127 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-170  T2CEP  WVir     7.683   239    3  5125   62  0.000  1000  0    
OGLE-LMC-T2CEP-171  T2CEP  BLHer    1.555   109    6  6375  562  0.000  1000  0    
OGLE-LMC-T2CEP-172  T2CEP  WVir    11.221   334   21  4875  250  0.000  1000  0    
OGLE-LMC-T2CEP-173  T2CEP  WVir     4.148    55    3  3900  112  0.000  1000  0    
OGLE-LMC-T2CEP-174  T2CEP  RVTau   46.819  6549  342  6000  438  1.333  1100  0  P=47.019 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-175  T2CEP  WVir     9.326   331    6  5250  125  0.000  1000  0    
OGLE-LMC-T2CEP-176  T2CEP  WVir     7.990   315    4  5375  125  0.000  1000  0    
OGLE-LMC-T2CEP-177  T2CEP  WVir    15.036   440   14  5000  188  0.000  1000  0    
OGLE-LMC-T2CEP-178  T2CEP  WVir    12.212   319   11  5000  188  0.000  1000  0    
OGLE-LMC-T2CEP-179  T2CEP  WVir     8.050   230    4  5000   62  0.000  1000  0    
OGLE-LMC-T2CEP-180  T2CEP  RVTau   30.996  3139  182  5500  500  1.467   700  0    
OGLE-LMC-T2CEP-181  T2CEP  pWVir    7.213   427   24  5375  312  0.000  1000  0    
OGLE-LMC-T2CEP-182  T2CEP  WVir     8.226   372    9  5250  125  0.000  1000  0  P=8.240 [1998AJ....115.1921A]  
OGLE-LMC-T2CEP-183  T2CEP  WVir     6.510   145    8  4625  125  0.000  1000  0    
OGLE-LMC-T2CEP-184  T2CEP  WVir    14.840   309   16  4625  188  0.000  1000  0    
OGLE-LMC-T2CEP-185  T2CEP  WVir    12.688  1842   33  4625   62  0.000  1000  0    
OGLE-LMC-T2CEP-186  T2CEP  WVir    16.362   519   16  4875  125  0.000  1000  0    
OGLE-LMC-T2CEP-187  T2CEP  BLHer    2.404    96    4  5500  375  0.000  1000  0    
OGLE-LMC-T2CEP-188  T2CEP  BLHer    1.049    87    4  6125  375  0.000  1000  0    
OGLE-LMC-T2CEP-189  T2CEP  BLHer    1.308    79    2  6250  125  0.000  1000  0    
OGLE-LMC-T2CEP-190  T2CEP  RVTau   38.362  2450   56  5625  188  0.019   700  0    
OGLE-LMC-T2CEP-191  T2CEP  RVTau   34.345  3969  127  5750  250  1.251   700  0    
OGLE-LMC-T2CEP-192  T2CEP  RVTau   26.194   916   32  5375  250  0.000  1000  0    
OGLE-LMC-T2CEP-193  T2CEP  WVir     7.005   273    4  5250   62  0.000  1000  0    
OGLE-LMC-T2CEP-194  T2CEP  BLHer    1.314   101    5  6375  250  0.000  1000  0    
OGLE-LMC-T2CEP-195  T2CEP  BLHer    2.753   141    5  5875  312  0.000  1000  0    
OGLE-LMC-T2CEP-196  T2CEP  WVir    14.958   668   20  5125  188  0.000  1000  0    
OGLE-LMC-T2CEP-197  T2CEP  BLHer    1.224    96    7  6375  438  0.000  1000  0    
OGLE-LMC-T2CEP-198  T2CEP  RVTau   38.274   908   32  4500  125  0.000  1000  0    
OGLE-LMC-T2CEP-199  T2CEP  RVTau   37.204  7090  338  8600  300  0.024  1000  0    
OGLE-LMC-T2CEP-200  T2CEP  RVTau   34.917  1695  114  4875  375  1.158   700  0    
OGLE-LMC-T2CEP-201  T2CEP  pWVir   11.007  2172   84  6500  250  0.150   180  0    
OGLE-LMC-T2CEP-202  T2CEP  RVTau   38.136  1028   24  4625  125  0.000  1000  0    
OGLE-LMC-T2CEP-203  T2CEP  RVTau   37.127   887   36  4625  188  0.000  1000  0    
OGLE-SMC-ACEP-01    ANCEP  1O       0.621   118    3  7250  188  0.000  1000  0    
OGLE-SMC-ACEP-02    ANCEP  F        0.828    78    1  6125   62  0.000  1000  0    
OGLE-SMC-ACEP-03    ANCEP  1O       0.570   103    3  7125  250  0.000  1000  0    
OGLE-SMC-ACEP-04    ANCEP  F        0.830   100    1  6375  125  0.000  1000  0    
OGLE-SMC-ACEP-05    ANCEP  1O       0.521    99    2  7000  125  0.000  1000  0    
OGLE-SMC-ACEP-06    ANCEP  F        1.256   167   10  6875  250  0.000  1000  0    
OGLE-SMC-T2CEP-001  T2CEP  pWVir   11.869  2570  102  6250  125  0.000  1000  0    
OGLE-SMC-T2CEP-002  T2CEP  BLHer    1.372   109    4  6750  312  0.000  1000  0    
OGLE-SMC-T2CEP-003  T2CEP  WVir     4.360   173    7  5875  312  0.000  1000  0    
OGLE-SMC-T2CEP-004  T2CEP  WVir     6.533   299   14  5375  375  0.000  1000  0    
OGLE-SMC-T2CEP-005  T2CEP  WVir     8.206   282    3  5375   62  0.000  1000  0    
OGLE-SMC-T2CEP-006  T2CEP  BLHer    1.236    80    1  6375   62  0.000  1000  0    
OGLE-SMC-T2CEP-007  T2CEP  RVTau   30.961  7560 1970  6125  750  0.000  1000  0    
OGLE-SMC-T2CEP-008  T2CEP  BLHer    1.490   117    2  5875  125  0.000  1000  0    
OGLE-SMC-T2CEP-009  T2CEP  BLHer    2.971   151    3  5625  125  0.000  1000  0    
OGLE-SMC-T2CEP-010  T2CEP  pWVir   17.481  4264  319  6000  312  0.000  1000  0    
OGLE-SMC-T2CEP-011  T2CEP  pWVir    9.925  3758  136  7250  250  0.028  1000  0    
OGLE-SMC-T2CEP-012  T2CEP  RVTau   29.219  1301   41  5375   62  0.000  1000  0    
OGLE-SMC-T2CEP-013  T2CEP  WVir    13.810   478   13  5375   62  0.000  1000  0    
OGLE-SMC-T2CEP-014  T2CEP  WVir    13.878   426    8  5375   62  0.000  1000  0    
OGLE-SMC-T2CEP-015  T2CEP  BLHer    2.570   458   21  7500  312  0.000  1000  0    
OGLE-SMC-T2CEP-016  T2CEP  BLHer    2.113   122    3  6000  188  0.000  1000  0    
OGLE-SMC-T2CEP-017  T2CEP  BLHer    1.299   115    5  6375  375  0.000  1000  0    
OGLE-SMC-T2CEP-018  T2CEP  RVTau   39.519  3539  166  5875  375  1.616  1200  0    
OGLE-SMC-T2CEP-019  T2CEP  RVTau   40.912  3481  101  6250  125  0.037   598  1    
OGLE-SMC-T2CEP-020  T2CEP  RVTau   50.623  1885   84  5375  188  0.000  1000  0     
OGLE-SMC-T2CEP-021  T2CEP  BLHer    2.313    94    1  6000  125  0.000  1000  0    
OGLE-SMC-T2CEP-022  T2CEP  BLHer    1.471    61    2  6000  250  0.000  1000  0    
OGLE-SMC-T2CEP-023  T2CEP  pWVir   17.675  1508   28  5750  125  0.000  1000  0  EB  
OGLE-SMC-T2CEP-024  T2CEP  RVTau   43.961  3075  126  6000  188  0.077   700  0    
OGLE-SMC-T2CEP-025  T2CEP  pWVir   14.171   941   34  5750  125  0.000  1000  0    
OGLE-SMC-T2CEP-026  T2CEP  BLHer    1.705   153    2  6375  125  0.000  1000  0    
OGLE-SMC-T2CEP-027  T2CEP  BLHer    1.542    81    2  6250  125  0.000  1000  0    
OGLE-SMC-T2CEP-028  T2CEP  pWVir   15.264  1854   53  5375   62  0.000  1000  0  EB  
OGLE-SMC-T2CEP-029  T2CEP  RVTau   33.676  6273  157  5375   62  0.000  1000  0  EB  
OGLE-SMC-T2CEP-030  T2CEP  BLHer    3.389   418    9  6750  188  0.000  1000  0    
OGLE-SMC-T2CEP-031  T2CEP  WVir     7.895   323   21  5375  312  0.000  1000  0    
OGLE-SMC-T2CEP-032  T2CEP  WVir    14.247   693   30  5750  188  0.086   600  0    
OGLE-SMC-T2CEP-033  T2CEP  BLHer    1.878   198    6  6375  188  0.000  1000  0    
OGLE-SMC-T2CEP-034  T2CEP  WVir    20.121   994   39  5375   62  0.000  1000  0    
OGLE-SMC-T2CEP-035  T2CEP  WVir    17.181   730   31  5500  312  0.025  1100  0    
OGLE-SMC-T2CEP-036  T2CEP  BLHer    1.092   141    2  6500  125  0.000  1000  0    
OGLE-SMC-T2CEP-037  T2CEP  BLHer    1.559   127    3  6125  125  0.000  1000  0    
OGLE-SMC-T2CEP-038  T2CEP  pWVir    4.444   734   32  6500  250  0.000  1000  0    
OGLE-SMC-T2CEP-039  T2CEP  BLHer    1.888   142    1  5875   62  0.000  1000  0    
OGLE-SMC-T2CEP-040  T2CEP  WVir    16.111   662   64  5375  312  0.000  1000  0    
OGLE-SMC-T2CEP-041  T2CEP  RVTau   29.118  1393   49  5750  125  0.000  1000  0    
OGLE-SMC-T2CEP-042  T2CEP  BLHer    1.487   100    2  6250   62  0.000  1000  0    
OGLE-SMC-T2CEP-043  T2CEP  RVTau   23.743  1285   57  5375  125  0.000  1000  0 W3 excess  

